Look Around and Learn: Self-Training Object Detection by Exploration

When an object detector is deployed in a novel setting it often experiences a drop in performance. This paper studies how an embodied agent can automatically fine-tune a pre-existing object detector while exploring and acquiring images in a new environment without relying on human intervention, i.e., a fully self-supervised approach. In our setting, an agent initially learns to explore the environment using a pre-trained off-the-shelf detector to locate objects and associate pseudo-labels. By assuming that pseudo-labels for the same object must be consistent across different views, we learn the exploration policy Look Around to mine hard samples, and we devise a novel mechanism called Disagreement Reconciliation for producing refined pseudo-labels from the consensus among observations. We implement a unified benchmark of the current state-of-the-art and compare our approach with pre-existing exploration policies and perception mechanisms. Our method is shown to outperform existing approaches, improving the object detector by 6.2% in a simulated scenario, a 3.59% advancement over other state-of-the-art methods, and by 9.97% in the real robotic test without relying on ground-truth. Code for the proposed approach and baselines are available at https://iit-pavis.github.io/Look_Around_And_Learn/.

==> preamble.tex <==
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\gs}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\usepackage{tabularx,multirow,booktabs}
\usepackage{scalerel}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{array}
\usepackage{pifont}
\usepackage{comment}
\usepackage{bm}
\usepackage{newunicodechar}
\usepackage{graphicx}
\newunicodechar{�}{\includegraphics{eyes}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\pname}{\textit{Disagreement Reconciliation}\xspace}
\newcommand{\aname}{\textit{Look Around}\xspace}
\newcommand{\baname}{\textbf{Look Around}\xspace}

